CATO: End-to-End Optimization of ML-Based Traffic Analysis Pipelines

Machine learning has shown tremendous potential for improving the capabilities of network traffic analysis applications, often outperforming simpler rule-based heuristics. However, ML-based solutions remain difficult to deploy in practice. Many existing approaches only optimize the predictive performance of their models, overlooking the practical challenges of running them against network traffic in real time. This is especially problematic in the domain of traffic analysis, where the efficiency of the serving pipeline is a critical factor in determining the usability of a model. In this work, we introduce CATO, a framework that addresses this problem by jointly optimizing the predictive performance and the associated systems costs of the serving pipeline. CATO leverages recent advances in multi-objective Bayesian optimization to efficiently identify Pareto-optimal configurations, and automatically compiles end-to-end optimized serving pipelines that can be deployed in real networks. Our evaluations show that compared to popular feature optimization techniques, CATO can provide up to 3600x lower inference latency and 3.7x higher zero-loss throughput while simultaneously achieving better model performance.

==> applications.tex <==
\section{Experimental Setup}
Because we include microbenchmarks to motivate \sysname, we introduce our
experimental setup now. We present two traffic analysis use cases that we use as
running examples throughout the paper: application service classification and
IoT device classification. Both of these are general machine learning
classification tasks and are representative of common traffic analysis tasks
that would be deployed against network traffic in real time.

\vspace{5pt} \noindent \textbf{Application Service Identification.}\quad While
there are many open data sources for network traces, none are able to be
replayed at or near 100~Gbps without repetition in a way that can properly
stress test ML-based traffic analysis in a high-speed traffic
scenario~\cite{retina}. As a result, we develop our own use case that identifies
one of six common application services (e.g., Netflix, Zoom, etc.) from a large
university network using network and transport layer flow statistics, labeled
using the server name exposed in the TLS handshake. This type of traffic
analysis task is typically used by web application firewalls and as an early
stage in network QoE inference pipelines~\cite{waf, qoe}. Models are trained
offline and deployed in the same network to classify services in real-time. We
note that while using live traffic from a large network allows us to run
experiments at line rate, real traffic is inherently inconsistent and difficult
to control or reproduce. We combat this by running experiments temporally close
to each other and running multiple trials where possible.

\vspace{5pt} \noindent \textbf{IoT Device Classification.}\quad To help with
reproducibility, we introduce an IoT device classification use case that assigns
IoT device labels to observed network connections. As in~\cite{n3ic}, we focus
on a 10-class classification task that labels each connection with one of nine
possible device categories, or ``other''. Models are trained offline and
evaluated offline using a set of packet traces. We use the traces published
by~\cite{iotclass}. 

\vspace{5pt} \noindent \textbf{Experimental Platform.}\quad Unless otherwise
stated, all experiments were conducted on a single server. The machines used in
our experiments run Ubuntu 20.04 and contain 384 GB of memory and a 100~GbE
Mellanox ConnectX-5 NIC. The server used for live traffic experiments contains a
dual Xeon Gold 6248R 3GHz CPU, while the server used for offline experiments
contains a dual Xeon Gold 6154 3GHz CPU.

\vspace{5pt} \noindent \textbf{Ethical Considerations.}\quad As part of our
experiments with high-speed network traffic, we performed measurements using a
tap on our campus network. We collected aggregate layer 3 and layer 4 flow
statistics features along with an application name derived from the SNI in TLS
handshakes (see Appendix~\ref{app:features} for the full list of features). We
did not investigate human behavior, store packets to disk, or view any
individual records or IP addresses. We restricted all live traffic experiments
to the server connected to the network tap, and the tap setup only saw a copy of
traffic to prevent impact on network users in the event of a system failure. The
server used was deployed in partnership with our campus networking and security
teams.



